Aspects of Thermal QCD Phenomenology at Intermediate Gauge/'t Hooft Coupling from String/M-Theory, (HD) Gravity Islands, and Multiverse

As applications of arXiv:2004.07259, the first part of the thesis is based on (i) arXiv:2011.04660 wherein we computed the low energy coupling constants of SU(3) chiral perturbation theory at NLO in the chiral expansion in the chiral limit, from the type IIA string dual inclusive of ${\cal O}(R^4)$ corrections and found a novel HD-large-$N$ connection; (ii) arXiv:2108.05372, arXiv:2203.11959 wherein we discussed confinement-deconfinement phase transition in thermal QCD-like theories at intermediate coupling in the absence/presence of rotation and observed (a) a novel "UV-IR" mixing, (b) "Flavor Memory" effect, (c) M$\chi$PT compatibility,(d) non-renormalization of deconfinement temperature $T_c$ beyond one loop in the zero instanton sector, and (e) found that the $T_c$ of rotating QGP decreases when angular velocity of rotating cylindrical black hole increases and vice-versa. In the second part of thesis, we obtained Page curves of Reissner-Nordstr\"{o}m black holes in the presence of ${\cal O}(R^2)$ terms and black holes with multiple horizons in arXiv:2204.11882 and arXiv:2210.00331 respectively. In arXiv:2207.04048, we constructed a doubly holographic setup for a non-conformal bath (thermal QCD) in ${\cal M}$-theory background with the inclusion of ${\cal O}(R^4)$ terms and obtained the Page curve of an eternal neutral black hole for massless graviton localized on an ETW-"brane"/(Fluxed) hypersurface. Multiverse is described as the setup of 2n anti de-Sitter (AdS) or de-Sitter branes embedded in the corresponding bulk (arXiv:2301.06151). Since all the universes can communicate with each other due to transparent boundary conditions at the defect, therefore one could exchange information between any universes. This setup is also used to obtain the Page curve of the Schwarzschild de-Sitter black hole, which has two horizons.

==> Hawking.tex <==
\newpage
~\\
~\\
~\\
~\\
~\\
~\\
~\\
~\\
~\\
\thispagestyle{empty}
%\begin{flushright}
\begin{center}
\large{{\it \textbf{``HOWEVER DIFFICULT LIFE MAY SEEM, THERE IS ALWAYS SOMETHING YOU CAN DO AND SUCCEED AT. IT MATTERS THAT YOU DON'T JUST GIVE UP.''}}}~\\
\large{\bf \hspace{3.5in} ~ STEPHEN HAWKING}
\end{center}
%\end{flushright}
\clearpage
\addtocounter{page}{-1}


==> pubs.tex <==
%Satyam Shivam Sundaram
%Jai Mata Di
%\newpage
\pagestyle{plain}
%\addtocounter{page}{1}
\begin{center}
{\large{\bf \underline{List of Publications}}}
\end{center}

This thesis contains the research works done in ``holographic thermal QCD'' (Part-I) and ``black hole information paradox'' (Part-II). List of the publications are given as following.


\begin{itemize}
\item {\bf Part-{\bf I} is based on the top-down holographic study of thermal QCD at intermediate coupling and includes the following papers.}
\begin{enumerate}
\item Vikas~Yadav, {\bf Gopal~Yadav} and Aalok~Misra, {\it (Phenomenolology/Lattice-Compatible) $SU(3)$ M$\chi$PT HD up to ${\cal O}(p^4)$ and the ${\cal O}(R^4)$-Large-N Connection}, JHEP {\bf 08} (2021) 151 [arXiv:2011.04660[hep-th]].

\item {\bf Gopal~Yadav}, Vikas~Yadav and Aalok~Misra, {\it ${\cal {M}}$cTEQ (${\cal {M}}$ {\bf c}hiral perturbation theory-compatible deconfinement {\bf T}emperature and {\bf E}ntanglement Entropy up to terms {\bf Q}uartic in curvature) and FM ({\bf F}lavor {\bf M}emory)}, JHEP {\bf 10} (2021) 220 [arXiv:2108.05372[hep-th]].

\item {\bf Gopal~Yadav}, {\it Deconfinement Temperature of Rotating QGP at Intermediate Coupling from ${\cal M}$-Theory}, Phys. Lett. B {\bf 841} (2023) 137925 [arXiv:2203.11959[hep-th]].
\end{enumerate}
\item {\bf Part-{\bf II} is based on the black hole information paradox and written on the basis of the papers listed below.}
\begin{enumerate}
\item {\bf Gopal~Yadav}, {\it Page Curves of Reissner-Nordstr{\"o}m Black Hole in HD Gravity}, Eur. Phys. J. C {\bf 82} (2022) 904 [arXiv:2204.11882[hep-th]].

\item {\bf Gopal~Yadav} and Aalok~Misra, {\it Entanglement entropy and Page curve from the ${\cal M}$-theory dual of thermal QCD above $T_c$ at intermediate coupling}, Phys. Rev. D {\bf 107} (2023) 10, 106015 [arXiv:2207.04048[hep-th]].

\item {\bf Gopal~Yadav} and Nitin~Joshi, {\it Cosmological and black hole islands in multi-event horizon spacetimes}, Phys. Rev. D {\bf 107}, 026009 (2023) [arXiv:2210.00331[hep-th]].

\item {\bf Gopal~Yadav}, {\it Multiverse in Karch-Randall Braneworld}, JHEP {\bf 03} (2023) 103 [arXiv:2301.06151[hep-th]].
\end{enumerate}

\item {\bf The papers which are not included in thesis are listed below}.
\begin{enumerate}
\item Aalok~Misra and {\bf Gopal~Yadav}, {\it (Almost) Contact (3) (Metric) Structure(s) and Transverse $SU(3)$ Structures Associated with ${\cal M}$-Theory Dual of Thermal QCD at Intermediate Coupling}, under review [arXiv:2211.13186[hep-th]].

\item Aalok~Misra and {\bf Gopal~Yadav}, {\it QCD-Compatible Supermassive Inert Top-Down Holographic Mesinos at Intermediate Coupling}, under review [arXiv:2308.05033[hep-th]].

\end{enumerate}

\end{itemize}


%\newpage
%{\large{\bf \underline{Schools:}}}

%\begin{enumerate}
%\item {{\it An International School and Conference on Functional Materials (ISCFM-2011)} during  March 28 - April 3, 2011 at Harish Chandra Research
%Institute, Allahabad, India.}
%\end{enumerate}
%\newpage


